Autonomous Overtaking in Gran Turismo Sport Using Curriculum Reinforcement Learning

Professional race-car drivers can execute extreme overtaking maneuvers. However, existing algorithms for autonomous overtaking either rely on simplified assumptions about the vehicle dynamics or try to solve expensive trajectory-optimization problems online. When the vehicle approaches its physical limits, existing model-based controllers struggle to handle highly nonlinear dynamics, and cannot leverage the large volume of data generated by simulation or real-world driving. To circumvent these limitations, we propose a new learning-based method to tackle the autonomous overtaking problem. We evaluate our approach in the popular car racing game Gran Turismo Sport, which is known for its detailed modeling of various cars and tracks. By leveraging curriculum learning, our approach leads to faster convergence as well as increased performance compared to vanilla reinforcement learning. As a result, the trained controller outperforms the built-in model-based game AI and achieves comparable overtaking performance with an experienced human driver.

==> images/human-vs-best-agent-overtaking-ver2.tex <==
% This file was created by tikzplotlib v0.9.4.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Traveling Time (sec)},
xmajorgrids,
xmin=-2, xmax=102,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Number of Cars overtook},
ymajorgrids,
ymin=-0.25, ymax=5.25,
ytick style={color=black}
]
\addplot [only marks, mark=*, draw=color0, fill=color0, opacity=0.9, colormap/viridis, forget plot]
table{%
x                      y
0 0
15 1
21.9 2
39.5 3
57.216 4
96.772 5
};
\addplot [only marks, mark=*, draw=red, fill=red, opacity=0.9, colormap/viridis, forget plot]
table{%
x                      y
0 0
15.4 1
16.4 2
27.466 3
43.533 4
76.466 5
};
\path [fill=color0, fill opacity=0.6]
(axis cs:55.816,0)
--(axis cs:55.816,5)
--(axis cs:56.216,5)
--(axis cs:56.216,0)
--(axis cs:55.816,0)
--cycle;

\path [fill=color0, fill opacity=0.6]
(axis cs:58.516,0)
--(axis cs:58.516,5)
--(axis cs:58.816,5)
--(axis cs:58.816,0)
--(axis cs:58.516,0)
--cycle;

\path [fill=red, fill opacity=0.6]
(axis cs:74.733,0)
--(axis cs:74.733,5)
--(axis cs:74.866,5)
--(axis cs:74.866,0)
--(axis cs:74.733,0)
--cycle;

\addplot [thick, color0, opacity=0.9]
table {%
0 0
10.4 0
10.4 0.0196898999999974
10.5 0.0479080499999981
10.6 0.0735534499999971
10.7 0.0973175000000026
10.8 0.119085699999999
10.9 0.139080799999999
11 0.15753785
11.1 0.174987799999997
11.2 0.193542450000001
11.3 0.2136505
11.4 0.234750350000002
11.5 0.254699699999998
11.6 0.2739014
11.7 0.292999300000002
11.8 0.311996450000004
11.9 0.331127950000001
12 0.350451699999996
12.1 0.369723499999998
12.2 0.388812249999995
12.3 0.407607999999999
12.4 0.426629650000001
12.5 0.445758050000001
12.6 0.464593500000001
12.7 0.483285499999999
12.8 0.5020691
12.9 0.520559700000001
13 0.538717649999995
13.1 0.5569031
13.2 0.574771099999998
13.3 0.5921875
13.4 0.60910035
13.5 0.6255585
13.6 0.642346150000003
13.7 0.659408550000001
13.8 0.676040649999999
13.9 0.692190549999998
14 0.707540899999998
14.1 0.722305299999999
14.2 0.738467399999996
14.3 0.760467549999998
14.4 0.790295399999997
14.5 0.828051750000003
14.6 0.868719449999998
14.7 0.910412600000001
14.8 0.953784200000001
14.9 0.998440549999998
15.3 1
15.3 1.0858032
15.4 1.169516
15.5 1.2496979
15.6 1.3214081
15.7 1.3818268
15.8 1.43284305
15.9 1.47531435
16 1.5087463
16.1 1.5370514
16.2 1.56192625
16.3 1.5837677
16.4 1.604303
16.5 1.62325745
16.6 1.6393982
16.7 1.6524353
16.8 1.66317445
16.9 1.6718933
17 1.67901305
17.1 1.6853729
17.2 1.69112855
17.3 1.6964264
17.4 1.70149535
17.5 1.70620725
17.6 1.7107605
17.7 1.7156586
17.8 1.7209839
17.9 1.7266266
18 1.73203125
18.1 1.736792
18.2 1.7427307
18.3 1.7491882
18.4 1.75641785
18.5 1.764328
18.6 1.77240905
18.7 1.78062745
18.8 1.78847045
18.9 1.7960419
19 1.80358585
19.1 1.81085815
19.2 1.81794435
19.3 1.8251465
19.4 1.8322662
19.5 1.83934635
19.6 1.846405
19.7 1.85363155
19.8 1.86272885
19.9 1.8722626
20 1.88167115
20.1 1.8908569
20.2 1.8996918
20.3 1.90840455
20.4 1.91696775
20.5 1.92531734999999
20.6 1.93358155
20.7 1.94188845
20.8 1.95038755
20.9 1.95692749999999
21 1.96175235
21.1 1.9665161
21.2 1.9711792
21.3 1.97576295
21.4 1.9802765
21.5 1.98480225000001
21.6 1.98917845
21.7 1.99343265
21.8 1.99769285
36.5 2
36.5 2.00620115
36.6 2.04486695000001
36.7 2.08392335
36.8 2.12319335
36.9 2.1614746
37 2.19937135
37.1 2.23676145000001
37.2 2.27312625000001
37.3 2.3082886
37.4 2.34277955
37.5 2.37680055
37.6 2.4098755
37.7 2.44211425
37.8 2.47358400000001
37.9 2.50435180000001
38 2.53490599999999
38.1 2.56524655000001
38.2 2.5952087
38.3 2.62497559999999
38.4 2.65582275
38.5 2.6875671
38.6 2.71935425
38.7 2.7513855
38.8 2.78343504999999
38.9 2.81519165
39 2.8468262
39.1 2.87824705
39.2 2.90947265
39.3 2.9404663
39.4 2.97125245
50.2 3
50.2 3.00174559999998
50.3 3.01135254999999
50.4 3.02070315000001
50.5 3.02969970000001
50.6 3.03808595
50.7 3.04554444999999
50.8 3.05214845
50.9 3.0584595
51 3.06495359999999
51.1 3.07169190000002
51.2 3.07847899999999
51.3 3.0854736
51.4 3.09205320000001
51.5 3.09852294999998
51.6 3.10510254999999
51.7 3.11218265
51.8 3.12159425
51.9 3.13570555000001
52 3.15527345
52.1 3.17611085000001
52.2 3.19522704999999
52.3 3.21141359999999
52.4 3.23193359999998
52.5 3.25814205000002
52.6 3.28876955000001
52.7 3.31746825
52.8 3.34376219999999
52.9 3.37042234999999
53 3.39989014999999
53.1 3.43004150000002
53.2 3.45856934999999
53.3 3.48942870000001
53.4 3.52291260000002
53.5 3.55560304999999
53.6 3.5855591
53.7 3.6131836
53.8 3.63869630000001
53.916 3.66560059999999
54.016 3.6852783
54.116 3.70227049999999
54.216 3.71728515
54.316 3.73360594999999
54.416 3.7505249
54.516 3.76500245
54.616 3.77742920000001
54.716 3.78758545000001
54.816 3.79562989999999
54.916 3.80250245
55.016 3.8092529
55.116 3.8170044
55.216 3.82623289999999
55.316 3.84234620000002
55.416 3.85895995000001
55.516 3.87558590000001
55.616 3.89211424999999
55.716 3.90729979999999
55.816 3.91527100000001
55.916 3.9215332
56.016 3.92775879999999
56.116 3.9338745
56.216 3.93979495000001
56.316 3.94570314999999
56.416 3.95164795000001
56.516 3.95839845
56.616 3.96444095000002
56.716 3.9709961
56.816 3.9778198
56.916 3.9845703
57.016 3.9911255
57.116 3.9975952
91.472 4
91.472 4.03323055
91.572 4.07982025
91.672 4.12508085
91.772 4.1703476
91.872 4.2151871
91.972 4.2578888
92.072 4.29963685
92.172 4.34062805
92.272 4.37718965
92.372 4.407457
92.472 4.4325775
92.572 4.4542877
92.672 4.4723175
92.772 4.4900253
92.872 4.50921935
92.972 4.5275925
93.072 4.54253695
93.172 4.5547104
93.272 4.56477665
93.372 4.5735901
93.472 4.58173215
93.572 4.58943175
93.672 4.60002745
93.772 4.6159927
93.872 4.6315155
93.972 4.64719235
94.072 4.66328125
94.172 4.67906495
94.272 4.69470215
94.372 4.710202
94.472 4.7251038
94.572 4.74001465
94.672 4.75553895
94.772 4.7728485
94.872 4.7853943
94.972 4.79782105
95.072 4.8100067
95.172 4.8218872
95.272 4.8338989
95.372 4.8458832
95.472 4.857724
95.572 4.8697113
95.672 4.8813324
95.772 4.8928833
95.872 4.904483
95.972 4.9160217
96.072 4.9273987
96.172 4.938681
96.272 4.9498901
96.372 4.96092835
96.472 4.97180785
96.572 4.98263245
96.672 4.9932434
};
\addlegendentry{Human Baseline}
\addplot [thick, red, opacity=0.9, dashed]
table {%
0 0
12.133 0
12.133 0.0152191000000016
12.2 0.0369842500000004
12.266 0.0586547500000052
12.333 0.0801849000000004
12.4 0.101516750000002
12.466 0.122674549999999
12.533 0.143627900000001
12.6 0.163928199999998
12.666 0.183517499999999
12.733 0.20281675
12.8 0.22182315
12.866 0.240509049999997
12.933 0.258926400000001
13 0.277227799999997
13.066 0.295376550000003
13.133 0.313449099999997
13.2 0.331460549999997
13.266 0.349307249999998
13.333 0.3669464
13.4 0.384298699999999
13.466 0.401342800000003
13.533 0.418264749999997
13.6 0.4352844
13.666 0.452380349999999
13.733 0.469396999999998
13.8 0.486175550000002
13.866 0.502667200000002
13.933 0.518945300000001
14 0.535064699999998
14.066 0.550967400000002
14.133 0.566854899999998
14.2 0.583749399999999
14.266 0.602487199999996
14.333 0.623159799999996
14.4 0.64656675
14.466 0.671243249999998
14.533 0.696218850000002
14.6 0.721350100000001
14.666 0.746408049999997
14.733 0.771069299999999
14.8 0.795516950000001
14.866 0.819982900000002
14.933 0.8444885
15 0.869003299999997
15.066 0.893490650000001
15.133 0.917950399999995
15.2 0.942422499999998
15.266 0.966876250000001
15.333 0.991204849999997
15.4 1
15.4 1.11056215
15.466 1.1843353
15.533 1.2564148
15.6 1.3262482
15.666 1.39393615
15.733 1.45984495
15.8 1.52479555
15.866 1.58872685
15.933 1.6518158
16 1.7137329
16.066 1.774411
16.133 1.8340454
16.2 1.8820862
16.266 1.9251953
16.333 1.96593015
20.133 2
20.133 2.0075043
20.2 2.02149355
20.266 2.0352844
20.333 2.049115
20.4 2.0629883
20.466 2.07668155
20.533 2.0901123
20.6 2.1033966
20.666 2.1164429
20.733 2.12925415
20.8 2.1418884
20.866 2.15441895
20.933 2.16691285000001
21 2.1792969
21.066 2.19151000000001
21.133 2.20275270000001
21.2 2.2139282
21.266 2.22490235
21.333 2.2357117
21.4 2.24628295
21.466 2.2566223
21.533 2.2670288
21.6 2.27736815
21.666 2.28742675000001
21.733 2.29714964999999
21.8 2.30656739999999
21.866 2.31583254999999
21.933 2.32499385
22 2.3339844
22.066 2.3426819
22.133 2.35107425
22.2 2.35931395
22.266 2.36746825
22.333 2.37543945
22.4 2.38324585
22.466 2.39160765
22.533 2.4008728
22.6 2.41103515000001
22.666 2.42124025000001
22.733 2.4311096
22.8 2.44083860000001
22.866 2.45061035
22.933 2.46040039999999
23 2.4700745
23.066 2.4795532
23.133 2.48875125
23.2 2.49747924999999
23.266 2.5058594
23.333 2.51425780000001
23.4 2.5227844
23.466 2.53132935
23.533 2.53955075
23.6 2.5487793
23.666 2.55841065000001
23.733 2.56815184999999
23.8 2.57772825
23.866 2.58714594999999
23.933 2.59647825
24 2.605896
24.066 2.61539305
24.133 2.62486574999999
24.2 2.63416139999999
24.266 2.6432312
24.333 2.6522949
24.4 2.6614746
24.466 2.6705078
24.533 2.67924805
24.6 2.6879761
24.666 2.69688110000001
24.733 2.7056824
24.8 2.7142273
24.866 2.7223755
24.933 2.7310303
25 2.73991090000001
25.066 2.74854124999999
25.133 2.75720215
25.2 2.7659912
25.266 2.7747803
25.333 2.78336794999999
25.4 2.79182735000001
25.466 2.8003113
25.533 2.80878295
25.6 2.81712645
25.666 2.8254944
25.733 2.83373415
25.8 2.841864
25.866 2.85007935
25.933 2.85825195
26 2.86629025000001
26.066 2.87445064999999
26.133 2.88164675
26.2 2.8887573
26.266 2.89569705
26.333 2.90244750000001
26.4 2.90913085000001
26.466 2.9157654
26.533 2.92233884999999
26.6 2.9287842
26.666 2.9351135
26.733 2.9413452
26.8 2.94749145000001
26.866 2.95357055000001
26.933 2.95952149999999
27 2.96537475
27.066 2.9711487
27.133 2.97682495
27.2 2.98234864999999
27.266 2.9878662
27.333 2.9934082
27.4 2.99885865
34 3
34 3.02904055
34.066 3.05842285
34.133 3.08531495
34.2 3.10900875
34.266 3.12957155
34.333 3.1476318
34.4 3.16330565
34.466 3.17633665
34.533 3.18882445
34.6 3.20088500000001
34.666 3.2128601
34.733 3.2253479
34.8 3.2376892
34.866 3.24885255
34.933 3.25919190000001
35 3.2687317
35.066 3.27729495
35.133 3.28469845
35.2 3.29139405000001
35.266 3.29768675
35.333 3.3032593
35.4 3.30782475
35.466 3.3117676
35.533 3.3159851
35.6 3.32057495
35.666 3.32568970000001
35.733 3.3312744
35.8 3.33672485000001
35.866 3.34196780000001
35.933 3.34711915
36 3.35235595
36.066 3.35770265
36.133 3.36317749999999
36.2 3.36883544999999
36.266 3.37463375
36.333 3.38048705
36.4 3.38643185000001
36.466 3.3925476
36.533 3.3985779
36.6 3.40445555
36.666 3.41034550000001
36.733 3.41632080000001
36.8 3.42230835
36.866 3.4281128
36.933 3.43395385
37 3.4399536
37.066 3.44636840000001
37.133 3.45297849999999
37.2 3.45964964999999
37.266 3.46621700000001
37.333 3.47265015
37.4 3.47908325000001
37.466 3.4856018
37.533 3.4920288
37.6 3.49835815
37.666 3.50477295000001
37.733 3.51136475000001
37.8 3.51796265
37.866 3.5244507
37.933 3.53093869999999
38 3.53746335000001
38.066 3.5439331
38.133 3.55023195
38.2 3.55654294999999
38.266 3.56298830000001
38.333 3.56953125
38.4 3.57614745000001
38.466 3.58273925000001
38.533 3.5892456
38.6 3.59562989999999
38.666 3.60200195
38.733 3.60838624999999
38.8 3.61484375
38.866 3.62132569999999
38.933 3.62764890000001
39 3.6338745
39.066 3.64025879999999
39.133 3.64666749999999
39.2 3.65286865
39.266 3.65898439999999
39.333 3.66522219999999
39.4 3.67142334999999
39.466 3.6774414
39.533 3.68341065
39.6 3.68957520000001
39.666 3.6958496
39.733 3.7020874
39.8 3.70823975000001
39.866 3.71427000000001
39.933 3.72020265000001
40 3.72609864999999
40.066 3.73204344999999
40.133 3.73790280000001
40.2 3.74367674999999
40.266 3.74951174999999
40.333 3.75550535
40.4 3.76141355
40.466 3.76705320000001
40.533 3.77253420000002
40.6 3.77806395
40.666 3.78406984999999
40.733 3.7901245
40.8 3.79602050000001
40.866 3.80185545000002
40.933 3.80773925000001
41 3.81359864999999
41.066 3.81936035000001
41.133 3.82513429999999
41.2 3.83096925
41.266 3.83670655000001
41.333 3.84234620000002
41.4 3.8479736
41.466 3.8536621
41.533 3.85924075
41.6 3.86470944999999
41.666 3.87016599999999
41.733 3.87558594999998
41.8 3.88111570000001
41.866 3.88653565
41.933 3.89189454999998
42 3.89726559999999
42.066 3.9026001
42.133 3.90772704999999
42.2 3.91278075
42.266 3.91788329999999
42.333 3.92283935
42.4 3.92768555
42.466 3.9325073
42.533 3.93734135
42.6 3.94206545
42.666 3.94663085
42.733 3.95129395000001
42.8 3.95596925
42.866 3.96053469999999
42.933 3.96501464999999
43 3.96944580000002
43.066 3.97386475000001
43.133 3.9783203
43.2 3.98280030000001
43.266 3.98728025
43.333 3.9916504
43.4 3.99571530000001
43.466 3.9994629
69.466 4
69.466 4.01473390000001
69.533 4.03316649999999
69.6 4.04963379999999
69.666 4.06417234999999
69.733 4.07683105000001
69.8 4.08762205
69.866 4.0987183
69.933 4.11094969999999
70 4.12408445000001
70.066 4.13797609999999
70.133 4.15288085
70.2 4.16868900000002
70.266 4.18245850000001
70.333 4.19422605
70.4 4.20422365000002
70.466 4.21251220000002
70.533 4.21917725000001
70.6 4.22429199999999
70.666 4.22801509999999
70.733 4.23404539999999
70.8 4.24195555000001
70.866 4.25008545000001
70.933 4.25900879999999
71 4.26888429999999
71.066 4.2780884
71.133 4.28476559999999
71.2 4.29144285
71.266 4.29810795000001
71.333 4.30480955
71.4 4.31136475000001
71.466 4.3177124
71.533 4.32373050000001
71.6 4.3293457
71.666 4.33454589999999
71.733 4.33925784999999
71.8 4.34348144999999
71.866 4.34724120000001
71.933 4.35069579999999
72 4.35396725000001
72.066 4.35723874999999
72.133 4.36058345000001
72.2 4.36408690000001
72.266 4.36765135000001
72.333 4.37075200000002
72.4 4.37092284999999
72.466 4.3712158
72.533 4.37177735
72.6 4.37344970000001
72.666 4.37871090000001
72.733 4.38663329999999
72.8 4.39682614999999
72.866 4.40749515
72.933 4.41861574999998
73 4.43000490000002
73.066 4.44143064999998
73.133 4.45275880000001
73.2 4.46573490000001
73.266 4.4805664
73.333 4.49719235
73.4 4.51451420000001
73.466 4.5310669
73.533 4.54742429999999
73.6 4.56368404999998
73.666 4.57987059999998
73.733 4.59576415000001
73.8 4.6111206
73.866 4.62595215000001
73.933 4.64051514999999
74 4.6548706
74.066 4.66906740000002
74.133 4.68303225
74.2 4.69674075
74.266 4.71042480000001
74.333 4.7239014
74.4 4.73714600000001
74.466 4.74995114999999
74.533 4.7621948
74.6 4.77373044999999
74.666 4.7845703
74.733 4.79490965
74.8 4.79689940000001
74.866 4.79626464999999
74.933 4.79573975000001
75 4.7953125
75.066 4.79471434999998
75.133 4.79404294999999
75.2 4.79332274999999
75.266 4.79261475000001
75.333 4.79254149999999
75.4 4.79406735
75.466 4.79782714999999
75.533 4.80460204999999
75.6 4.81495359999999
75.666 4.8281982
75.733 4.84245604999999
75.8 4.8571289
75.866 4.87211915
75.933 4.8873779
76 4.90225829999999
76.066 4.91602785
76.133 4.92924805
76.2 4.94296875
76.266 4.95811765000001
76.333 4.9753418
76.4 4.99545899999998
};
\addlegendentry{Our Agent (Best)}
\addplot [color0, opacity=0.8, forget plot]
table {%
56.016 0
56.016 5
};
\addplot [color0, opacity=0.8, forget plot]
table {%
58.666 0
58.666 5
};
\addplot [red, opacity=0.8, dashed, forget plot]
table {%
74.7995 0
74.7995 5
};
\end{axis}

\end{tikzpicture}


==> sections/preliminary.tex <==
\section{Preliminaries}

\subsection{Reinforcement Learning}
Reinforcement learning~(RL) can be formulated using an infinite-horizon Markov Decision Process~(MDP) 
defined by a tuple $(\mathcal{S}, \mathcal{A}, \mathcal{P}, r, \rho_0, \gamma)$~\cite{sutton1998reinforcement}.
The RL agent starts in a state~$\bs{s}_t \in \mathcal{S}$
drawn from an initial state distribution $\rho_0(\bs{s})$.
At every time step, an action $\bs{a}_t \in \mathcal{A}$ sampled
from a stochastic policy $\pi(\bs{a}_t|\bs{s}_t)$ is executed
and the agent transitions to the next state~$\bs{s}_{t+1}$
with the state transition probability~$\mathcal{P}^{\bs{a}_t}_{\bs{s}_t\bs{s}_{t+1}}
	= \text{Pr}( \bs{s}_{t+1} | \bs{s}_t, \bs{a}_t)$,
receiving an immediate reward~${r(\bs{s}_t, \bs{a}_t)\in\mathbb{R}}$.
The goal of standard RL is to find an optimal 
policy~$\pi^\ast$ that maximizes the expected reward.

% \begin{equation} \label{eq: rl_obj1}
%     \pi^{\ast} = \arg \max_{\pi} \mathbb{E}_{\bs{\tau} \sim \pi} \left[ \sum_{t=0}^{\infty} \gamma^t r(\bs{s}_t, \bs{a}_t) \right]
% \end{equation}
% where $\bs{\tau} = (\bs{s}_t, \bs{a}_t, r_t)$ is a sampled trajectory using the policy $\pi$
% and $\gamma \in (0, 1)$ as discount factor.
% Here, $r_t$ is the reward function which formulates the task.
  
% \subsection{Soft Actor-Critic}
Soft actor-critic~(SAC) is an off-policy maximum entropy deep reinforcement learning
algorithm~\cite{haarnoja2018soft} that maximizes an entropy-regularized objective:
\begin{equation}
    \max_{\bs{\theta}} \quad J(\bs{\theta}) = \sum_{t=1}^{T} \mathbb{E}_{(\bs{s}_t, \bs{a}_t)\sim\rho_{\pi}} 
    [ r(\bs{s}_t, \bs{a}_t) + \alpha \mathcal{H}\left( \pi_{\bs{\theta}}(\cdot | \bs{s}_t) \right)]
\end{equation}
where $\alpha$ is a temperature parameter that trades off between maximizing 
the policy entropy $\mathcal{H}$~(exploration) and the reward~(exploitation).
% 
Hence, it simultaneously maximizes expected return while exploring as much as possible.  
% 
SAC has been shown to be an effective deep RL algorithm due to several key properties, 
such as the entropy-regularized objective, off-policy training, and state-dependent exploration. 

\subsection{Curriculum Learning}
The basic idea behind curriculum learning~(CL) is very intuitive---start solving a small problem, 
and then gradually increase the problem complexity. 
In~\cite{elman1993learning}, the author first demonstrated the importance of incorporating such a learning 
strategy into neural networks training for a simple language grammar task. 
Although RL came later to exploring the potential of CL, several lines of research have explored 
how tasks can be sequenced into a curriculum for learning a complicated problem that may otherwise
be too difficult to learn from scratch~\cite{narvekar2020curriculum}. 


==> tables/evaluation_policies.tex <==
\begin{table}[h]
\caption{Evaluate different training strategies.}
\label{tab-evaluation-policies}
\begin{center}
\begin{small}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{c||c|c}
\toprule
\rowcolor{Gray}
 & Training Procedure & Training Epochs   \\
\midrule
 Agent1    & 2 stages & [500, 500] \\
\midrule
 Agent2   & 3 stages (\NEW{small collision penalty})    & [500, 500, 500] \\
\midrule
 Agent3 & 3 stages (\NEW{large collision penalty})  & [500, 500, 500] \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\end{table}

==> tables/evaluation_settings.tex <==
\begin{table}[h]
\caption{Evaluation Settings}
\label{tab-evaluation-settings}
\begin{center}
\begin{small}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{|c||c|c|c|c|}
\hline
\multirow{2}{2.5em}{Setting} & Initial & Number of  & \multirow{2}{4em}{Race Car} & \multirow{2}{5em}{Race Track} \\
                           & Distance &  Cars &                             &                          \\
\hline
\hline
 A & 50m  &      5       & \multirow{2}{4em}{Audi TT Cup ’16} & Tokyo Expressway  \\
\cline{1-3}
 B & 200m &     5         &                             & Central Outer Loop\\
\hline
\end{tabular}
\end{small}
\end{center}
\end{table}
